Data optimizations for constraint automata

Constraint automata (CA) constitute a coordination model based on finite automata on infinite words. Originally introduced for modeling of coordinators, an interesting new application of CAs is implementing coordinators (i.e., compiling CAs into executable code). Such an approach guarantees correctness-by-construction and can even yield code that outperforms hand-crafted code. The extent to which these two potential advantages materialize depends on the smartness of CA-compilers and the existence of proofs of their correctness. Every transition in a CA is labeled by a "data constraint" that specifies an atomic data-flow between coordinated processes as a first-order formula. At run-time, compiler-generated code must handle data constraints as efficiently as possible. In this paper, we present, and prove the correctness of two optimization techniques for CA-compilers related to handling of data constraints: a reduction to eliminate redundant variables and a translation from (declarative) data constraints to (imperative) data commands expressed in a small sequential language. Through experiments, we show that these optimization techniques can have a positive impact on performance of generated executable code.

==> cmds.tex <==
%\let\oldcurlyvee\curlyvee
%\renewcommand{\curlyvee}[1][]	{\oldcurlyvee_{\!#1}}

%\newcommand{\nil}{\textsf{\upshape\small nil}}
\newcommand{\cmdskip}{\texttt{\upshape skip}}
\newcommand{\cmdasgn}{\mathbin{\texttt{\upshape:=}}}
\newcommand{\cmdseq}{\mathbin{\texttt{\upshape;}}}
\newcommand{\cmdifthen}[2]{\texttt{\upshape if}\;#1\;\texttt{\upshape then}\;#2\;\texttt{\upshape fi}}
\newcommand{\cmdifthenf}[2]{\texttt{\upshape if}\;#1\;\texttt{\upshape ->}\;#2\;\texttt{\upshape fi}}
\newcommand{\cmduniv}{\mathbb{C}\mathsc{md}}

%\newcommand{\confuniv}{\mathbb{C}\mathsc{onf}}

\newcommand{\tripuniv}{\mathbb{T}\mathsc{riple}}

%\newcommand{\fail} {\textsf{\upshape fail}}


\newcommand{\asrtand}		{\mathrel{\textbf{\upshape\&}}} % {\mathrel{\blacktriangle}}
\newcommand{\asrtmodels}	{\models_\text{\upshape tot}}
\newcommand{\asrtuniv}		{\mathbb{A}\mathsc{srt}}

\newcommand{\modelstot}	{\models_\text{\upshape tot}}

\newcommand{\termnil}		{\code{nil}}


\newcommand{\fununiv}		{\mathbb{F}\mathsc{un}}
%\newcommand{\funiv}	{\mathbb{F}}

\newcommand{\arityfun}	{\textsf{\upshape arity}}

%\newcommand{\duniv}	{\mathbb{D}}
%\newcommand{\runiv}	{\mathbb{R}}
\newcommand{\reluniv}	{\mathbb{R}\mathsc{el}}

\newcommand{\at}[1]	{\code{d}_{#1}} % {\langle#1\rangle}

\newcommand{\nilfreefun}	{\termnil\textsf{\upshape-Free}}
\newcommand{\argfun}	{\textsf{\upshape Arg}}

\newcommand{\deltai}{\delta_\text{init}}

%\newcommand{\bprec} {\blacktriangleleft}

\newcommand{\proves} {\vdash}
\newcommand{\provestot} {\vdash_{\text{\upshape tot}}}

%\newcommand{\termeq}		{\approx} % {\mathrel{\texttt{=}}}
%\newcommand{\termuniv}	{\mathbb{T}\mathsc{erm}}
%
%\newcommand{\freefun}	{\textsf{\upshape Free}}

%\newcommand{\bgraph} {\textsc{b}-graph\xspace}
%\newcommand{\bgraphs} {\textsc{b}-graphs\xspace}
%\newcommand{\barc} {\textsc{b}-arc\xspace}
%\newcommand{\barcs} {\textsc{b}-arcs\xspace}
%
%\newcommand{\puniv}	{\mathbb{P}}
%
%\newcommand{\evalfun} {\mathsf{eval}}

\newcommand{\precond}		{\mathsf{Pre}}
\newcommand{\postcond}		{\mathsf{Post}}
\newcommand{\interm}		{\mathsf{Interm}}
\newcommand{\invar}			{\mathsf{Inv}}
\newcommand{\cond}			{\mathsf{Cond}}

%\newcommand{\Assert}[1]		{\State \ensuremath{\color[HTML]{008000} \big\{ \begin{array}[t]{@{} l @{} l @{}} #1 & \big\}\end{array}}}
%
%\newcommand{\acc}			{{\downarrow}}

\newcommand{\cale}			{\mathcal{E}}
\newcommand{\calf}			{\mathcal{F}}
\newcommand{\cali}			{\mathcal{I}}
%\newcommand{\calm}			{\mathcal{M}}
%\newcommand{\calo}			{\mathcal{O}}
%\newcommand{\calp}			{\mathcal{P}}
\newcommand{\calt}			{\mathcal{T}}
\newcommand{\calv}			{\mathcal{V}}
\newcommand{\calw}			{\mathcal{W}}
%\newcommand{\calx}			{\mathcal{X}}
\newcommand{\caly}			{\mathcal{Y}}
\newcommand{\cauniv}		{\mathbb{CA}}
\newcommand{\cpfun}			{\mathsf{cp}}
\newcommand{\ceil}[3][]		{\mathrel{{\ifthenelse{\equal{#1}{}}{\longrightarrow}{\xrightarrow{\;#1\;}}} \lceil #2 / #3 \rceil}}
\newcommand{\charfun}		{\mathsf{Char}}
%\newcommand{\co}[1]			{\overline{#1}}
\newcommand{\cocale}		{\overline{\mathcal{E}}}

\newcommand{\datauniv}		{\mathbb{D}\mathsc{ata}}
\newcommand{\dcand}			{\wedge}
%\newcommand{\dcbigand}			{\bigwedge}
\newcommand{\dcbot}			{\bot} % {\texttt{\upshape 0}}
\newcommand{\dcdfun}		{\texttt{\upshape d}}
\newcommand{\dceqpred}		{\texttt{\upshape Eq}}
%\newcommand{\dcequiv}		{\mathrel{\equiv_\text{\upshape dc}}}
%\newcommand{\dcfun}			{\mathsf{DC}}
%\newcommand{\dcmodels}		{\mathrel{\models^{\!\!\!\!\!^{_\text{\upshape dc}}}}}
\newcommand{\dcnot}			{\neg}
\newcommand{\dcor}			{\vee}
\newcommand{\dctop}			{\top} % {\texttt{\upshape 1}}
%\newcommand{\dcuniv}		{\mathbb{DC}}
\newcommand{\disuniv}		{\mathbb{D}\mathsc{istr}}

\newcommand{\edgefun}		{\mathsf{Edge}}
\newcommand{\esfun}			{\mathord{\begin{array}{@{}c@{}}\bigoplus\end{array}}}
\newcommand{\floor}[1][]	{\mathrel{\lfloor {\ifthenelse{\equal{#1}{}}{\longrightarrow}{\xrightarrow{\;#1\;}}} \rfloor}}
\newcommand{\graphuniv}		{\mathbb{G}\mathsc{raph}}
\newcommand{\graphfun}		{\mathsf{graph}}
\newcommand{\interp}[1]		{\llbracket #1 \rrbracket}
\newcommand{\interpx}[2][c]	{\left\llbracket \begin{array}{@{} #1 @{}} #2 \end{array} \right\rrbracket}
\newcommand{\langfun}		{\mathsf{Lang}}
\newcommand{\nscuniv}		{{\mathbb{NSC}}}
\newcommand{\nscfun}		{\mathsf{Nsc}}
\newcommand{\partitfun}		{{\bigstar}}
\newcommand{\pauniv}		{{\mathbb{PA}}}
\newcommand{\pfun}			{\mathord{\begin{array}{@{}c@{}}\prod\end{array}}} % {\mathrm{\Pi}}
\newcommand{\portuniv}		{{\mathbb{P}\mathsc{ort}}}
\newcommand{\portorder}		{\mathrel{<_\portuniv}}
%\newcommand{\portfun}[1][]	{\mathsf{Port}} % {\mathsf{Port\text{\footnotesize\sf #1}}}

%\newcommandtwoopt{\relr}[2][][]	{\mathrel{R_{#1}^{#2}}}
\newcommand{\runfun}		{\mathsf{Run}}
\newcommand{\rununiv}		{\mathbb{R}\mathsc{un}}

\newcommand{\scequiv}		{\mathrel{\equiv_\text{\upshape sc}}}
\newcommand{\scmodels}		{\mathrel{\models^{\!\!\!\!\!^{_\text{\upshape sc}}}}}
\newcommand{\scuniv}		{{\mathbb{SC}}}
\newcommand{\scorder}		{\mathrel{<_\scuniv}}
\newcommand{\scfun}			{\mathsf{SC}}
\newcommand{\sfun}			{\mathord{\begin{array}{@{}c@{}}\sum\end{array}}}
\newcommand{\spsfun}		{(\sfun \pfun \sfun)}
\newcommand{\stateuniv}		{\mathbb{S}\mathsc{tate}}
\newcommand{\streamuniv}	{\mathbb{S}\mathsc{tr}}
\newcommand{\trad}			{\mathsf{Trad}}
\newcommand{\tranuniv}		{\mathbb{T}\mathsc{ran}}
\newcommand{\tscfun}		{\mathsf{Tsc}}
\newcommand{\usim}			{\preceq}
\newcommand{\veruniv}		{\mathbb{V}\mathsc{er}}

\newcommand{\xprime}		{\mathrel{\vphantom{\rightarrow}}'}

%\newcommand{\BIP}		{\textsc{Bip}\xspace}
\newcommand{\CA}		{\textsc{ca}\xspace}
\newcommand{\CAs}		{\textsc{ca}s\xspace}
\newcommand{\CSP}		{\textsc{csp}\xspace}
\newcommand{\CSPs}		{\textsc{csp}s\xspace}
\newcommand{\DC}		{\textsc{dc}\xspace}
\newcommand{\DCs}		{\textsc{dc}s\xspace}
\newcommand{\DNF}		{\textsc{dnf}\xspace}
%\newcommand{\ECT}		{\textsc{Ect}\xspace}
%\newcommand{\IO}		{\textsc{i/o}\xspace}
%\newcommand{\MPI}		{\textsc{Mpi}\xspace}
\newcommand{\NSC}		{\textsc{nsc}\xspace}
\newcommand{\NSCs}		{\textsc{nsc}s\xspace}
\newcommand{\SC}		{\textsc{sc}\xspace}
\newcommand{\SCs}		{\textsc{sc}s\xspace}
\newcommand{\XML}		{\textsc{Xml}\xspace}

%\newcommand{\reo}[1]	{\ensuremath{\mathsf{#1}}}

%
% TIKZ - NODES
%

\newcommand{\tikzmixednode}{%
	\ifcompiletikz{%
		\begin{tikzpicture}[node distance=1.5cm]
			\node[reonode, minimum size=.25cm]	(N) [] {};
			\node[invis]						(I1) [left of=N] {};
			\node[invis]						(I2) [above=.6cm of I1] {};
			\node[invis]						(I3) [below=.6cm of I1] {};
			\node[invis]						(O1) [right of=N] {};
			\node[invis]						(O2) [above=.3cm of O1] {};
			\node[invis]						(O3) [below=.3cm of O1] {};

			\draw[sync, >-]	(N) to node {} (O2);
			\draw[sync, >-]	(N) to node {} (O3);
			\draw[sync]		(I1) to node {} (N);
			\draw[sync]		(I2) to node {} (N);
			\draw[sync]		(I3) to node {} (N);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzsinknode}{%
	\ifcompiletikz{%
		\begin{tikzpicture}[node distance=1.5cm]
			\node[reobnode, minimum size=.25cm]	(N) [] {};
			\node[invis]						(I1) [left of=N] {};
			\node[invis]						(I2) [above=.6cm of I1] {};
			\node[invis]						(I3) [below=.6cm of I1] {};

			\draw[sync]		(I1) to node {} (N);
			\draw[sync]		(I2) to node {} (N);
			\draw[sync]		(I3) to node {} (N);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzsourcenode}{%
	\ifcompiletikz{%
		\begin{tikzpicture}[node distance=1.5cm]
			\node[reobnode, minimum size=.25cm]	(N) [] {};
			\node[invis]						(O1) [right of=N] {};
			\node[invis]						(O2) [above=.6cm of O1] {};
			\node[invis]						(O3) [below=.6cm of O1] {};

			\draw[sync, >-]	(N) to node {} (O1);
			\draw[sync, >-]	(N) to node {} (O2);
			\draw[sync, >-]	(N) to node {} (O3);
		\end{tikzpicture}
	} \fi
}

%
% TIKZ - CHANNELS
%

\newcommand{\tikzchanfifo}[2]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[invis,label=above right:$\reo{#1}$]	(I) [] {};
			\node[invis,label=above left:$\reo{#2}$]	(O) [right of=I] {};

			\draw[fifo]	(I) to node {} (O);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzchanlsync}[2]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[invis,label=above right:$\reo{#1}$]	(I) [] {};
			\node[invis,label=above left:$\reo{#2}$]	(O) [right of=I] {};

			\draw[lossysync]	(I) to node {} (O);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzchansdrain}[2]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[invis,label=above right:$\reo{#1}$]	(I1) [] {};
			\node[invis,label=above left:$\reo{#2}$]	(I2) [right of=I1] {};

			\draw[syncdrain]	(I1) to node {} (I2);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzchansync}[2]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[invis,label=above right:$\reo{#1}$]	(I) [] {};
			\node[invis,label=above left:$\reo{#2}$]	(O) [right of=I] {};

			\draw[sync]	(I) to node {} (O);
		\end{tikzpicture}
	} \fi
}

%
% TIKZ - CONNECTORS
%

\newcommand{\tikzalternator}[3]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reobnode,label=left:$\reo{#2}$]	(B) [below of=A] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [right of=A] {};
			
			\draw[syncdrain] (A) to node {} (B);
			\draw[sync] (A) to node {} (C);
			\draw[fifo] (B) to node {} (C);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzalternatorii}[3]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reobnode,label=left:$\reo{#2}$]	(B) [below of=A] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [right of=A] {};
			\node[reonode]							(D) [right of=B] {};
			
			\draw[syncdrain] (A) to node {} (B);
			\draw[sync] (A) to node {} (C);
			\draw[sync] (B) to node {} (D);
			\draw[fifo] (D) to node {} (C);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzalternatoriii}[4]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reobnode,label=left:$\reo{#2}$]	(B) [below of=A] {};
			\node[reobnode,label=left:$\reo{#3}$]	(C) [below of=B] {};
			\node[reobnode,label=right:$\reo{#4}$]	(D) [right of=A] {};
			\node[reonode]							(E) [right of=B] {};
			\node[reonode]							(F) [right of=C] {};
			
			\draw[syncdrain] (A) to node {} (B);
			\draw[sync] (A) to node {} (D);
			\draw[syncdrain] (B) to node {} (C);
			\draw[sync] (B) to node {} (E);
			\draw[sync] (C) to node {} (F);
			\draw[fifo] (E) to node {} (D);
			\renewcommand{\buffername}{\ensuremath{y}}
			\draw[fifo] (F) to node {} (E);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzexampleconn}[5]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			
			\node[reonode,label=right:$\reo{#5}$]	(X) [] {};
			\node[reobnode,label=left:$\reo{#1}$]	(A) [above left of=X] {};
			\node[reobnode,label=left:$\reo{#2}$]	(B) [below left of=X] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [above right of=X] {};
			\node[reobnode,label=right:$\reo{#4}$]	(D) [below right of=X] {};
			
			\draw[sync] (A) to node {} (X);
			\draw[filter] (B) to node {} (X);
			\draw[fifo] (X) to node {} (C);
			\renewcommand{\buffername}{\ensuremath{y}}
			\draw[fifo] (X) to node {} (D);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzexclrouter}[6]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reonode,label=right:$\reo{#5}$]	(Y) [right of=A] {};
			\node[reonode,label=right:$\reo{#4}$]	(X) [above of=Y] {};
			\node[reonode,label=right:$\reo{#6}$]	(Z) [below of=Y] {};
			\node[reobnode,label=right:$\reo{#2}$]	(B) [right of=X] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [right of=Z] {};
			
			\draw[lossysync] (A) to node {} (X);
			\draw[syncdrain] (A) to node {} (Y);
			\draw[lossysync] (A) to node {} (Z);
			\draw[sync] (X) to node {} (Y);
			\draw[sync] (X) to node {} (B);
			\draw[sync] (Z) to node {} (Y);
			\draw[sync] (Z) to node {} (C);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzmerge}[3]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedisthalf]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[point]							(M) [below right of=A] {};
			\node[reobnode,label=left:$\reo{#2}$]	(B) [below left of=M] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [right of=M] {};
			
			\draw[channel]	(A) to node {} (M);
			\draw[channel]	(B) to node {} (M);
			\draw[sync]		(M) to node {} (C);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikznodenm}[7]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedisthalf]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[point]							(M1) [below right of=A] {};
			\node[reobnode,label=left:$\reo{#2}$]	(B) [below left of=M1] {};
			\node[reonode,label=above:$\reo{#3}$]	(C) [right of=M1] {};
			\node[point]							(M2) [below right of=C] {};
			\node[reobnode,label=left:$\reo{#4}$]	(D) [below left of=M2] {};
			\node[reonode,label=above:$\reo{#5}$]	(E) [right of=M2] {};
			\node[point]							(M3) [right of=E] {};
			\node[reobnode,label=right:$\reo{#6}$]	(F) [above right of=M3] {};
			\node[reobnode,label=right:$\reo{#7}$]	(G) [below right of=M3] {};
			
			\draw[channel]	(A) to node {} (M1);
			\draw[channel]	(B) to node {} (M1);
			\draw[sync]		(M1) to node {} (C);
			\draw[channel]	(C) to node {} (M2);
			\draw[channel]	(D) to node {} (M2);
			\draw[sync]		(M2) to node {} (E);
			\draw[channel]	(E) to node {} (M3);
			\draw[sync]		(M3) to node {} (F);
			\draw[sync]		(M3) to node {} (G);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzrepl}[3]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedisthalf]
			\node[reobnode,label=right:$\reo{#2}$]	(B) [] {};
			\node[point]							(M) [below left of=B] {};
			\node[reobnode,label=left:$\reo{#1}$]	(A) [left of=M] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [below right of=M] {};
			
			\draw[channel]	(A) to node {} (M);
			\draw[sync]		(M) to node {} (B);
			\draw[sync]		(M) to node {} (C);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzreplmerge}[5]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reobnode,label=right:$\reo{#2}$]	(B) [right of=A] {};
			\node[reobnode,label=left:$\reo{#3}$]	(C) [below of=A] {};
			\node[reobnode,label=right:$\reo{#4}$]	(D) [right of=C] {};
			\node[point] (AC) [below of=A, node distance=\tikznodedisthalf] {};
			\node[point] (BD) [below of=B, node distance=\tikznodedisthalf] {};
			\node[reonode,label=below:$\reo{#5}$]	(E) [right of=AC, node distance=\tikznodedisthalf] {};
			
 			\draw[sync] (A) to node {} (C);
 			\draw[sync] (B) to node {} (D);
 			\draw[sync] (AC) to node {} (E);
 			\draw[channel] (E) to node {} (BD);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzsyncsdrain}[3]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reonode,label=right:$\reo{#2}$]	(B) [right of=A] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [below of=B] {};
			
			\draw[sync] (A) to node {} (B);
			\draw[syncdrain] (B) to node {} (C);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzsyncfifo}[3]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reonode,label=right:$\reo{#2}$]	(B) [right of=A] {};
			\node[reobnode,label=right:$\reo{#3}$]	(C) [below of=B] {};
			
			\draw[sync] (A) to node {} (B);
			\draw[fifo] (B) to node {} (C);
		\end{tikzpicture}
	} \fi
}

\newcommand{\tikzsyncsync}[4]{%
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=\tikznodedist]
			\node[reobnode,label=left:$\reo{#1}$]	(A) [] {};
			\node[reobnode,label=right:$\reo{#2}$]	(B) [right of=A] {};
			\node[reobnode,label=left:$\reo{#3}$]	(C) [below of=A,node distance=.5cm] {};
			\node[reobnode,label=right:$\reo{#4}$]	(D) [right of=C] {};
			
 			\draw[sync] (A) to node {} (B);
 			\draw[sync] (C) to node {} (D);
		\end{tikzpicture}
	} \fi
}

%
% TIKZ - AUTOMATA
%

\newcommand{\tikzautone}[3]{%
	\newcommand{\n}{\protect \\}
	\ifcompiletikz{%
		\scalebox{1}{\begin{tikzpicture}[baseline]
			\node[state, initleft] (Q) {};
			
			\ifthenelse{\equal{#1}{}}{}{%
				\path[->] (Q) edge [trans, out=105, in=75, loop] node [above] {\scriptsize \LINES{#1}} (Q);
			}
			
			\ifthenelse{\equal{#2}{}}{}{%
				\path[->] (Q) edge [trans, out=15, in=-15, loop] node [right] {\scriptsize \LINES{#2}} (Q);
			}
			
			\ifthenelse{\equal{#3}{}}{}{%
				\path[->] (Q) edge [trans, out=-75, in=-105, loop] node [below] {\scriptsize \LINES{#3}} (Q);
			}
		\end{tikzpicture}}%
	}\fi%
}

\newcommand{\tikzautonee}[4]{%
	\newcommand{\n}{\protect \\}
	\ifcompiletikz{%
		\scalebox{1}{\begin{tikzpicture}[baseline]
			\node[state, pin={[pin edge={black, thick, <-}]above left:}] (Q) {};
			
			\ifthenelse{\equal{#1}{}}{}{%
				\path[->] (Q) edge [trans, out=105, in=75, loop] node [above] {\scriptsize \LINES{#1}} (Q);
			}
			
			\ifthenelse{\equal{#2}{}}{}{%
				\path[->] (Q) edge [trans, out=15, in=-15, loop] node [right] {\scriptsize \LINES{#2}} (Q);
			}
			
			\ifthenelse{\equal{#3}{}}{}{%
				\path[->] (Q) edge [trans, out=-75, in=-105, loop] node [below] {\scriptsize \LINES{#3}} (Q);
			}
			
			\ifthenelse{\equal{#4}{}}{}{%
				\path[->] (Q) edge [trans, out=-165, in=165, loop] node [left] {\scriptsize \LINES{#4}} (Q);
			}
		\end{tikzpicture}}%
	}\fi%
}

\newcommand{\tikzauttwo}[7]{%
	\newcommand{\n}{\protect \\}
	\ifcompiletikz{%
		\begin{tikzpicture}[baseline, node distance=.5*\tikznodedist, every text node part/.style={text centered}]
			\node[state, initleft] (Q) {};
			\node[state, right of=Q] (R) {};
			
			\ifthenelse{\equal{#1}{}}{}{%
				\path[->] (Q) edge [trans, out=120, in=60, loop] node [above] {\scriptsize \LINES{#1}} (Q);
			}
			
			\ifthenelse{\equal{#2}{}}{}{%
				\path[->] (Q) edge [trans, out=30, in=150] node [above] {\scriptsize \LINES{#2}} (R);
			}
			
			\ifthenelse{\equal{#3}{}}{}{%
				\path[->] (R) edge [trans, out=120, in=60, loop] node [above] {\scriptsize \LINES{#3}} (R);
			}
			
			\ifthenelse{\equal{#4}{}}{}{%
				\path[->] (R) edge [trans, out=30, in=-30, loop] node [right] {\scriptsize \LINES{#4}} (R);
			}
			
			\ifthenelse{\equal{#5}{}}{}{%
				\path[->] (R) edge [trans, out=-60, in=-120, loop] node [below] {\scriptsize \LINES{#5}} (R);
			}
			
			\ifthenelse{\equal{#6}{}}{}{%
				\path[->] (R) edge [trans, out=-150, in=-30] node [below] {\scriptsize \LINES{#6}} (Q);
			}
			
			\ifthenelse{\equal{#7}{}}{}{%
				\path[->] (Q) edge [trans, out=-60, in=-120, loop] node [below] {\scriptsize \LINES{#7}} (Q);
			}
		\end{tikzpicture}%
	}\fi
}

%
% TIKZ - GRAPHS
%

\newcommand{\tikzgraphmerger}[1]{%
	\ifthenelse{\equal{#1}{1}}{%
		\begin{tikzpicture}[baseline]
			\node (v1) at (0,1) {};
			\node (v2) at (0,0) {};
			\node (v3) at (0,-1) {};
			\node (v4) at (1.5,0) {};
			
			\begin{scope}[fill opacity=0.5]
				\filldraw[fill=cyan!50] ($(v1)+(-.25,0)$)
					to [out=90, in=180] ($(v1)+(0,.25)$)
					to [out=0, in=180] ($(v4)+(0,.25)$)
					to [out=0, in=90] ($(v4)+(.25,0)$)
					to [out=270, in=0] ($(v4)+(0,-.25)$)
					to [out=180, in=0] ($(v1)+(0,-.25)$)
					to [out=180, in=270] ($(v1)+(-.25,0)$);
					
				\filldraw[fill=magenta!50] ($(v2)+(-.25,0)$)
					to [out=90, in=180] ($(v2)+(0,.25)$)
					to [out=0, in=180] ($(v4)+(0,.35)$)
					to [out=0, in=90] ($(v4)+(.35,0)$)
					to [out=270, in=0] ($(v4)+(0,-.35)$)
					to [out=180, in=0] ($(v2)+(0,-.25)$)
					to [out=180, in=270] ($(v2)+(-.25,0)$);
					
				\filldraw[fill=yellow!50] ($(v3)+(-.25,0)$)
					to [out=90, in=180] ($(v3)+(0,.25)$)
					to [out=0, in=180] ($(v4)+(0,.45)$)
					to [out=0, in=90] ($(v4)+(.45,0)$)
					to [out=270, in=0] ($(v4)+(0,-.45)$)
					to [out=180, in=0] ($(v3)+(0,-.25)$)
					to [out=180, in=270] ($(v3)+(-.25,0)$);
			\end{scope}
			
			\fill (v1) node [anchor=west,inner sep=0pt] {\!\!\reo{A}};
			\fill (v2) node [anchor=west,inner sep=0pt] {\!\!\reo{B}};
			\fill (v3) node [anchor=west,inner sep=0pt] {\!\!\reo{C}};
			\fill (v4) node {\reo{Z}};
		\end{tikzpicture}%
	}{\ifthenelse{\equal{#1}{2}}{%
		\begin{tikzpicture}[baseline]
			\node (v1) at (0,1) {};
			\node (v2) at (0,0) {};
			\node (v4) at (1.5,0) {};
			
			\begin{scope}[fill opacity=0.5]
				\filldraw[fill=cyan!50] ($(v1)+(-.25,0)$)
					to [out=90, in=180] ($(v1)+(0,.25)$)
					to [out=0, in=180] ($(v4)+(0,.25)$)
					to [out=0, in=90] ($(v4)+(.25,0)$)
					to [out=270, in=0] ($(v4)+(0,-.25)$)
					to [out=180, in=0] ($(v1)+(0,-.25)$)
					to [out=180, in=270] ($(v1)+(-.25,0)$);
					
				\filldraw[fill=yellow!50] ($(v2)+(-.25,0)$)
					to [out=90, in=180] ($(v2)+(0,.25)$)
					to [out=0, in=180] ($(v4)+(0,.35)$)
					to [out=0, in=90] ($(v4)+(.35,0)$)
					to [out=270, in=0] ($(v4)+(0,-.35)$)
					to [out=180, in=0] ($(v2)+(0,-.25)$)
					to [out=180, in=270] ($(v2)+(-.25,0)$);
			\end{scope}
			
			\fill (v1) node [anchor=west,inner sep=0pt] {\!\!\reo{A}};
			\fill (v2) node [anchor=west,inner sep=0pt] {\!\!$\reo{B} , \reo{C}$};
			\fill (v4) node {\reo{Z}};
		\end{tikzpicture}%
	}{\ifthenelse{\equal{#1}{3}}{%
		\begin{tikzpicture}[baseline]
			\node (v2) at (0,0) {};
			\node (v4) at (1.5,0) {};
			
			\begin{scope}[fill opacity=0.5]
				\filldraw[fill=yellow!50] ($(v2)+(-.25,0)$)
					to [out=90, in=180] ($(v2)+(0,.25)$)
					to [out=0, in=180] ($(v4)+(0,.25)$)
					to [out=0, in=90] ($(v4)+(.25,0)$)
					to [out=270, in=0] ($(v4)+(0,-.25)$)
					to [out=180, in=0] ($(v2)+(0,-.25)$)
					to [out=180, in=270] ($(v2)+(-.25,0)$);
			\end{scope}
			
			\fill (v2) node [anchor=west,inner sep=0pt] {\!\!$\reo{A} , \reo{B} , \reo{C}$};
			\fill (v4) node {\reo{Z}};
		\end{tikzpicture}%
	}{%
	}}}
}

\newcommand{\tikzgraphhglass}[1]{%
	\ifthenelse{\equal{#1}{1}}{%
		\begin{tikzpicture}[baseline]
			\node (v1) at (-1.5,1) {};
			\node (v2) at (0,0) {};
			\node (v3) at (1.5,1) {};
			\node (v4) at (-1.5,-1) {};
			\node (v5) at (1.5,-1) {};
			
			\begin{scope}[fill opacity=0.5]
				\filldraw[fill=black!50] ($(v1)+(-.25,0)$)
					to [out=90, in=180] ($(v1)+(0,.25)$)
					to [out=0, in=180] ($(v3)+(0,.25)$)
					to [out=0, in=90] ($(v3)+(.25,0)$)
					to [out=270, in=0] ($(v3)+(0,-.25)$)
					to [out=180, in=90] ($(v2)+(.25,0)$)
					to [out=270, in=0] ($(v2)+(0,-.25)$)
					to [out=180, in=270] ($(v2)+(-.25,0)$)
					to [out=90, in=0] ($(v1)+(0,-.25)$)
					to [out=180, in=270] ($(v1)+(-.25,0)$);
				
				\filldraw[fill=cyan!50] ($(v1)+(-.35,0)$)
					to [out=90, in=180] ($(v1)+(0,.35)$)
					to [out=0, in=180] ($(v2)+(0,.35)$)
					to [out=0, in=180] ($(v5)+(0,.25)$)
					to [out=0, in=90] ($(v5)+(.25,0)$)
					to [out=270, in=0] ($(v5)+(0,-.25)$)
					to [out=180, in=0] ($(v2)+(0,-.35)$)
					to [out=180, in=0] ($(v1)+(0,-.35)$)
					to [out=180, in=270] ($(v1)+(-.35,0)$);
				
				\filldraw[fill=magenta!50] ($(v4)+(-.25,0)$)
					to [out=90, in=180] ($(v4)+(0,.25)$)
					to [out=0, in=270] ($(v2)+(-.45,0)$)
					to [out=90, in=180] ($(v2)+(0,.45)$)
					to [out=0, in=90] ($(v2)+(.45,0)$)
					to [out=270, in=180] ($(v5)+(0,.35)$)
					to [out=0, in=90] ($(v5)+(.35,0)$)
					to [out=270, in=0] ($(v5)+(0,-.35)$)
					to [out=180, in=0] ($(v4)+(0,-.25)$)
					to [out=180, in=270] ($(v4)+(-.25,0)$);
				
				\filldraw[fill=yellow!50] ($(v4)+(-.35,0)$)
					to [out=90, in=180] ($(v4)+(0,.35)$)
					to [out=0, in=180] ($(v2)+(0,.55)$)
					to [out=0, in=180] ($(v3)+(0,.35)$)
					to [out=0, in=90] ($(v3)+(.35,0)$)
					to [out=270, in=0] ($(v3)+(0,-.35)$)
					to [out=180, in=0] ($(v2)+(0,-.55)$)
					to [out=180, in=0] ($(v4)+(0,-.35)$)
					to [out=180, in=270] ($(v4)+(-.35,0)$);
			\end{scope}
			
			\fill (v1) node [anchor=west,inner sep=-3pt] {\reo{A}};
			\fill (v2) node {\reo{H}};
			\fill (v3) node [anchor=west,inner sep=-3pt] {\reo{Y}};
			\fill (v4) node [anchor=west,inner sep=-3pt] {\reo{B}};
			\fill (v5) node [anchor=west,inner sep=-3pt] {\reo{Z}};
		\end{tikzpicture}%
	}{\ifthenelse{\equal{#1}{2}}{%
		\begin{tikzpicture}[baseline]
			\node (v1) at (-1.5,1) {};
			\node (v2) at (0,0) {};
			\node (v3) at (1.5,1) {};
			\node (v4) at (-1.5,-1) {};
			\node (v5) at (1.5,-1) {};
			\node (v7) at (1.5,0) {};
			
			\begin{scope}[fill opacity=0.5]
				\filldraw[fill=black!50] ($(v1)+(-.25,0)$)
					to [out=90, in=180] ($(v1)+(0,.25)$)
					to [out=0, in=180] ($(v3)+(0,.25)$)
					to [out=0, in=90] ($(v3)+(.25,0)$)
					to [out=270, in=0] ($(v3)+(0,-.25)$)
					to [out=180, in=90] ($(v2)+(.25,0)$)
					to [out=270, in=0] ($(v2)+(0,-.25)$)
					to [out=180, in=270] ($(v2)+(-.25,0)$)
					to [out=90, in=0] ($(v1)+(0,-.25)$)
					to [out=180, in=270] ($(v1)+(-.25,0)$);
				
				\filldraw[fill=cyan!50] ($(v1)+(-.35,0)$)
					to [out=90, in=180] ($(v1)+(0,.35)$)
					to [out=0, in=180] ($(v2)+(0,.35)$)
					to [out=0, in=180] ($(v5)+(0,.25)$)
					to [out=0, in=90] ($(v5)+(.25,0)$)
					to [out=270, in=0] ($(v5)+(0,-.25)$)
					to [out=180, in=0] ($(v2)+(0,-.35)$)
					to [out=180, in=0] ($(v1)+(0,-.35)$)
					to [out=180, in=270] ($(v1)+(-.35,0)$);
				
				\filldraw[fill=yellow!50] ($(v4)+(-.25,0)$)
					to [out=90, in=180] ($(v4)+(0,.25)$)
					to [out=0, in=180] ($(v2)+(0,.45)$)
					to [out=0, in=180] ($(v7)+(0,.35)$)
					to [out=0, in=90] ($(v7)+(.35,0)$)
					to [out=270, in=0] ($(v7)+(0,-.35)$)
					to [out=180, in=0] ($(v2)+(0,-.45)$)
					to [out=180, in=0] ($(v4)+(0,-.25)$)
					to [out=180, in=270] ($(v4)+(-.25,0)$);
			\end{scope}
			
			\fill (v1) node [anchor=west,inner sep=-3pt] {\reo{A}};
			\fill (v2) node {\reo{H}};
			\fill (v3) node [anchor=east,inner sep=-3pt] {\reo{Y}};
			\fill (v4) node [anchor=west,inner sep=-3pt] {\reo{B}};
			\fill (v5) node [anchor=west,inner sep=-3pt] {\reo{Z}};
			\fill (v7) node [anchor=east,inner sep=-3pt] {\reo{Y}, \reo{Z}};
		\end{tikzpicture}%
	}{\ifthenelse{\equal{#1}{3}}{%
		\begin{tikzpicture}[baseline]
			\node (v1) at (-1.5,1) {};
			\node (v2) at (0,0) {};
			\node (v4) at (-1.5,-1) {};
			\node (v7) at (1.5,0) {};
			
			\begin{scope}[fill opacity=0.5]
				\filldraw[fill=cyan!50] ($(v1)+(-.25,0)$)
					to [out=90, in=180] ($(v1)+(0,.25)$)
					to [out=0, in=180] ($(v2)+(0,.25)$)
					to [out=0, in=180] ($(v7)+(0,.25)$)
					to [out=0, in=90] ($(v7)+(.25,0)$)
					to [out=270, in=0] ($(v7)+(0,-.25)$)
					to [out=180, in=0] ($(v2)+(0,-.25)$)
					to [out=180, in=0] ($(v1)+(0,-.25)$)
					to [out=180, in=270] ($(v1)+(-.25,0)$);
				
				\filldraw[fill=yellow!50] ($(v4)+(-.25,0)$)
					to [out=90, in=180] ($(v4)+(0,.25)$)
					to [out=0, in=180] ($(v2)+(0,.3	5)$)
					to [out=0, in=180] ($(v7)+(0,.35)$)
					to [out=0, in=90] ($(v7)+(.35,0)$)
					to [out=270, in=0] ($(v7)+(0,-.35)$)
					to [out=180, in=0] ($(v2)+(0,-.35)$)
					to [out=180, in=0] ($(v4)+(0,-.25)$)
					to [out=180, in=270] ($(v4)+(-.25,0)$);
			\end{scope}
			
			\fill (v1) node [anchor=west,inner sep=-3pt] {\reo{A}};
			\fill (v2) node {\reo{H}};
			\fill (v4) node [anchor=west,inner sep=-3pt] {\reo{B}};
			\fill (v7) node [anchor=east,inner sep=-3pt] {\reo{Y}, \reo{Z}};
		\end{tikzpicture}%
	}{\ifthenelse{\equal{#1}{4}}{%
		\begin{tikzpicture}[baseline]
			\node (v2) at (0,0) {};
			\node (v6) at (-1.5,0) {};
			\node (v7) at (1.5,0) {};
			
			\begin{scope}[fill opacity=0.5]
				\filldraw[fill=yellow!50] ($(v6)+(-.25,0)$)
					to [out=90, in=180] ($(v6)+(0,.25)$)
					to [out=0, in=180] ($(v2)+(0,.25)$)
					to [out=0, in=180] ($(v7)+(0,.25)$)
					to [out=0, in=90] ($(v7)+(.25,0)$)
					to [out=270, in=0] ($(v7)+(0,-.25)$)
					to [out=180, in=0] ($(v2)+(0,-.25)$)
					to [out=180, in=0] ($(v6)+(0,-.25)$)
					to [out=180, in=270] ($(v6)+(-.25,0)$);
			\end{scope}
			
			\fill (v2) node {\reo{H}};
			\fill (v6) node [anchor=west,inner sep=-3pt] {\reo{A}, \reo{B}};
			\fill (v7) node [anchor=east,inner sep=-3pt] {\reo{Y}, \reo{Z}};
		\end{tikzpicture}%
	}{%
	}}}}
}
